CamP: Camera Preconditioning for Neural Radiance Fields

Neural Radiance Fields (NeRF) can be optimized to obtain high-fidelity 3D scene reconstructions of objects and large-scale scenes. However, NeRFs require accurate camera parameters as input -- inaccurate camera parameters result in blurry renderings. Extrinsic and intrinsic camera parameters are usually estimated using Structure-from-Motion (SfM) methods as a pre-processing step to NeRF, but these techniques rarely yield perfect estimates. Thus, prior works have proposed jointly optimizing camera parameters alongside a NeRF, but these methods are prone to local minima in challenging settings. In this work, we analyze how different camera parameterizations affect this joint optimization problem, and observe that standard parameterizations exhibit large differences in magnitude with respect to small perturbations, which can lead to an ill-conditioned optimization problem. We propose using a proxy problem to compute a whitening transform that eliminates the correlation between camera parameters and normalizes their effects, and we propose to use this transform as a preconditioner for the camera parameters during joint optimization. Our preconditioned camera optimization significantly improves reconstruction quality on scenes from the Mip-NeRF 360 dataset: we reduce error rates (RMSE) by 67% compared to state-of-the-art NeRF approaches that do not optimize for cameras like Zip-NeRF, and by 29% relative to state-of-the-art joint optimization approaches using the camera parameterization of SCNeRF. Our approach is easy to implement, does not significantly increase runtime, can be applied to a wide variety of camera parameterizations, and can straightforwardly be incorporated into other NeRF-like models.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> method_previous.tex <==


\subsection{previous}

A common and simple way to mitigate differences in magnitude is to re-parameterize the problem. The simplest example is to multiply the parameter by a scalar, e.g., the parameterization $f = f^0 + \Delta f$ can be changed to $f = f^0 + s\Delta f$ where $s$ is a large scalar. This change is equivalent to preconditioning the optimization problem  with diagonal preconditioner $\mat{P}^{-1}$ identical to the identity except for the coordinate corresponding to the focal length, which would take a value of $s$.

While effective, simple parameter-scaling preoconditioners are not able to decouple highly correlated coefficients in the parameterization. To design more comprehensive preconditioners for camera optimization, we study the sensitivity of the camera projection function $\varprojection(\varpoint;\varcamparam)$ to its input camera parameters.
In understanding this problem, it is useful to think about how it behaves locally around a point $\mat{\phi^0}$ in the camera parameter space. 





Consider the Taylor approximation of the projection function $\varprojection(\varpoint;\varcamparam) \approx \varprojection(\varpoint;\mat{\phi^0}) + \varjac_\varprojection(\varcamparam - \mat{\phi^0})$, where $\varjac_\varprojection \in \mathbb R^{2 \times k}$ is the Jacobian of the projection at point $\mat{\phi^0}$. 
Consider perturbations to the camera parameter sampled from a normal distribution $\vardeltacamparam\sim\mathcal{N}(\mat{0};\sigma^2 \mat{I})$, we compute the covariance of the projection $\mat{Z}(\vardeltacamparam) = \varprojection(\varpoint;\mat{\phi^0}+\vardeltacamparam)$ as:
\begin{align}
    \Sigma_\Pi &= {\E_{\vardeltacamparam}} \left[(\mat{Z} - \E[\mat{Z}])(\mat{Z}-\E[\mat{Z}])^\top \right] \approx \sigma^2 \varjac_\Pi\varjac_\Pi^\top
\end{align}
using the first-order Taylor approximation described above.

Our goal is to make the outputs of the projection similar in magnitude and decorrelated of each other . We can \emph{whiten} the outputs of the projection function to have identity covariance by applying the transform
\begin{align}
    \varprojection_w(x; \hat{\varcamparam}) = \varprojection(\mat{x}; \varwhiten \hat{\varcamparam})\,.
\end{align}
so that $\mat{\Sigma}_{\varprojection_w} = $
This is also called the Zero Component Analysis (ZCA) whitening transform~\cite{kessy2018optimal} or Mahalanobis transform, and we adopt it as the value of our preconditioner:
\begin{align}
    \varprecon = \varwhiten
    \Sigma_\Pi &= {\E_{\vardeltacamparam}} \left[(\mat{Z} - \E[\mat{Z}])(\mat{Z}-\E[\mat{Z}])^\top \right] \approx \varjac_\Pi\Sigma_{\updel\phi}\varjac_\Pi^\top
\end{align}

preconditioner $P^{-1}$


We compute the whitening transform using an eigendecomposition of the covariance: if $\varcovproj=\vareigQ\vareigL\vareigQ^\top$ then $\varcovproj^{-\onehalf} = \vareigQ^\top\vareigL^{-\onehalf} \vareigQ$, where $\vareigQ$ is the matrix of eigenvectors of $\varcovproj$ and $\Lambda$ is a diagonal matrix containing its eigenvalues.
With the Taylor approximation, we assume $\varprojection$ is roughly linear near $\mat{\phi^0}$, and thus can fold the whitening transform into the input of the projection:
\begin{align}
    \varprojection_w(\varpoint;\varcamparam) \approx \varprojection\left(\varpoint;\varwhiten(\varcamparam-\mat{\phi^0})+\mat{\phi^0}\right) 
\end{align}
Note that the whitened projection function $\varprojection_w$ is evaluated at a specific spatial point $\varpoint$ and parameter $\varcamparam$. In practice, we compute the expected covariance matrix over a distribution or set of points $\varpoint\in \varpoints$. For example, the points can be uniformly sampled in a bounding box or in the camera frustum.









In the previous section, we explored how we can whiten the effect of the projection function on a point $\varpoint$ for perturbations of each parameter $\varcamparam+\vardeltacamparam$. In this section, we describe how to use this whitening transform to \emph{precondition} the camera parameters when training a NeRF.

When considering changes to the camera parameters, we observe that the resulting change in the rendered image is similar to changes in the 3D to 2D projection. We propose to directly use the whitening transform of the projection to precondition the camera parameters during NeRF training. This can be seen as using the projection of a set of 3D points as a proxy objective to the main training objective of NeRF.

Given the covariance matrix of the projection function $\varcovproj$, we can re-parameterize the camera parameter using a preconditioner $P^{-1}=\varcovproj^{-\onehalf}$ as $\varcamparam = \varprecon\tilde\varcamparam$, such that we track the decorrelated camera parameters $\tilde\varcamparam$ during training. Our preconditioner can be seen as a zero-component analysis (ZCA) whitening transform~\cite{kessy2018optimal} or a Mahalanobis transform.



We visualize the absolute magnitudes of the preconditioner in \figref{fig:preconditioning}, which takes larger values for parameters that do not affect much the projection, such as the focal length (first element), and lower value for the one with most effect (sixth element).
We can use the preconditioned parameters to showcase the effects of the preconditioner on the renders, and visualize those in \figref{fig:preconditioning_with_precondition}.


Our final method optimizes the loss function $\varloss(B;\varmodelparam, \varcamparam)$ by substituting $\varcamparam$ by $\varprecon \varcamparamdecorrelated$, where $\varcamparamdecorrelated$ stands for the decorrelated camera parameters. Besides the matrix multiply with the preconditioner, there is no other change in our implementation, and we can use standard optimizers, such as Adam~\cite{kingma2014adam}.

Note that because we model all the camera parameters in the optimization structure as residuals w.r.t. the initial estimate, there is no need to invert the initial value through the preconditioner $P$, as it is $0$. 

We now summarize our method for preconditioning camera optimization. At initialization, our method samples 3D points for each camera using the view frustum, and computes the covariance matrix of the projection w.r.t. the camera parameters at the initial estimate. 
We then compute the preconditioning matrix for each camera $i$ and re-parameterize the camera parameters as $\varcamparam_i = \varprecon_i\varcamparamdecorrelated_i$ for optimization.
After optimization, we recover the final camera parameters as $\varcamparam^* = \varprecon_i \varcamparamdecorrelated^*$ where $*$ superscript refers to the final estimate of the parameter after optimization.



In practice, we add a small dampening parameter to the diagonals of the covariance matrix $\varcov$ in order to better condition the matrix before taking the inverse matrix square root. Note that this is especially important with lens distortion parameters, as very small changes in them dramatically affect the point projection.
\begin{align}
    \varprecon &= \left( \varcov + \lambda \diag(\varcov) + \mu \mat{I} \right)^{-\onehalf}\,,
\end{align}

\keunhong{TODO: Add details about intrinsic sharing}

